A Survey of Deep Learning for Low-Shot Object Detection

Object detection has achieved a huge breakthrough with deep neural networks and massive annotated data. However, current detection methods cannot be directly transferred to the scenario where the annotated data is scarce due to the severe overfitting problem. Although few-shot learning and zero-shot learning have been extensively explored in the field of image classification, it is indispensable to design new methods for object detection in the data-scarce scenario since object detection has an additional challenging localization task. Low-Shot Object Detection (LSOD) is an emerging research topic of detecting objects from a few or even no annotated samples, consisting of One-Shot Object Detection (OSOD), Few-Shot Object Detection (FSOD) and Zero-Shot Object Detection (ZSD). This survey provides a comprehensive review of LSOD methods. First, we propose a thorough taxonomy of LSOD methods and analyze them systematically, comprising some extensional topics of LSOD (semi-supervised LSOD, weakly-supervised LSOD, and incremental LSOD). Then, we indicate the pros and cons of current LSOD methods with a comparison of their performance. Finally, we discuss the challenges and promising directions of LSOD to provide guidance for future works.

==> figures/OVD_framework.tex <==
\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/graph6_OVD.pdf}\\
\caption{(a) Three stages of Open-Vocabulary Object Detection~(OVD). In the pre-training stage, OVD requires to learn a strong visual-semantic mapping function on a large dataset with multiple image-text pairs. In the training stage, OVD trains a zero-shot detector on the base dataset. In the test stage, OVD tests the model on the novel dataset. (b) $C_B$ denotes base classes, $C_N$ denotes novel classes, and $C_O$ denotes the overall classes in the pre-training stage of OVD~($C_B$ and $C_N$ are not intersected, while $C_O$ intersects with both $C_B$ and $C_N$).}
\label{fig:ovd_framework}
\end{figure}

==> figures/soc_OSOL_attention_methods.tex <==
\begin{figure}
\centering
\subfigure[CoAE, BHRL, ABA OSOL, ADA OSOL, AUG OSOL]{
    \begin{minipage}[t]{0.4\linewidth}
    \centering
    \includegraphics[width=6cm]{images/graph5_CoAE.pdf}
    %\caption{fig1}
    \end{minipage}%
}%
\subfigure[AIT, CAT, SaFT]{
    \begin{minipage}[t]{0.6\linewidth}
    \centering
    \includegraphics[width=7.5cm]{images/graph5_AIT_CAT.pdf}
    %\caption{fig2}
    \end{minipage}%
}%
\centering
\caption{\color{blue} Overview of attention-based integral feature aggregation methods in OSOD. Some methods~(CoAE, BHRL, ABA OSOL, ADA OSOL, AUG OSOL) use a non-local operation for integral feature aggregation, while some methods~(AIT, CAT, SaFT) use transformer to capture attention between query images and support images.}
\label{fig:osod_attention_methods}
\end{figure}

==> figures/soc_OSOL_concate_methods.tex <==
\begin{figure}
\centering
\subfigure[SiamMask~\cite{Ivan2018SiamMask}]{
    \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=6.5cm]{images/graph3_SiamMask.pdf}
    %\caption{fig1}
    \end{minipage}%
}%
\subfigure[OSCD~\cite{FuZ0S21} OSOLwT~\cite{Li2021OSODwF}]{
    \begin{minipage}[t]{0.55\linewidth}
    \centering
    \includegraphics[width=7cm]{images/graph3_OSCD.pdf}
    %\caption{fig2}
    \end{minipage}%
}%

\subfigure[FOC OSOL~\cite{Yang2021foc}]{
    \begin{minipage}[t]{\linewidth}
    \centering
    \includegraphics[width=8cm]{images/graph3_FOC_OSOD.pdf}
    %\caption{fig2}
    \end{minipage}%
}
\centering
\caption{\color{blue} Overview of concatenation-based integral feature aggregation methods in OSOD. OSCD and OSOLwT concatenate the query feature map with the pooled embedding vector of the support feature map. SiamMask concatenates the query feature map with the absolute difference between the query feature map and the pooled embedding vector of the support feature map instead. FOC OSOL additionally applies convolution blocks on the integral feature map generated in SiamMask.}
\label{fig:osol_concate_methods}
\end{figure}

==> figures/soc_ZSOD_base_novel_relation.tex <==
\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/ZSD-base-novel-super.pdf}\\
\caption{\color{blue} Illustration of semantic relation methods: \textbf{base-novel class relation} and \textbf{super-class relation}. Methods based on base-novel class relation utilize semantic similarities between base classes and novel classes to transfer knowledge from base classes to novel classes~(these methods are categorized into \textbf{linear-transform-based methods} and \textbf{graph-based methods}). Methods based on super-class relation assume that there is a hierarchical relationship among categories, and they utilize this hierarchical relationship to assist prediction. Note that $C_B$ and $C_N$ denote the number base classes and novel classes, respectively.}
% \textbf{(1)} denotes TOPM-ZSOD\cite{shao2019zero}, \textbf{(2)} denotes LSA-ZSOD~\cite{wang2020learning}, \textbf{(3)} denotes DPIF~\cite{li2021inference}, and $\otimes$ denotes the matrix multiplication.
% TOPM-ZSOD~\cite{shao2019zero}, LSA-ZSOD~\cite{wang2020learning}, DPIF~\cite{li2021inference}
\label{fig:zsod_base_novel_super}
\end{figure}

==> n04_extensional_FSOD.tex <==
\section{Extensional Few-Shot Object Detection\label{sec:non_standard_fsod_methods}}

\subsection{Semi-Supervised Few-Shot Object Detection\label{sec:semi_fsod_methods}}

\noindent $\bullet$ \textbf{WL-FSOD}~\cite{MisraSHWatchAndLearn15}. Semi-supervised Few-Shot Object Detection~(semi-supervised FSOD) aims to utilize abundant unlabeled data to assist FSOD.
WL-FSOD is an early method that conducts semi-supervised FSOD on a large video dataset. WL-FSOD adopts traditional Exemplar-SVM~\cite{Tomasz2011Exemplar} as the detection framework which is different from later deep-learning-based detectors. This method iteratively excavates the potential objects from the unlabeled dataset with a uLSIF algorithm~\cite{Kana2009uLSIF} to decrease the predicted false-positive samples. Further, it uses the weighted flow within the bounding box and the trellis graph across frames to tackle the failure modes of object tracking.
This method is an early semi-supervised FSOD method based on the traditional detector, which has unsatisfying performance but it still inspires later methods in this area.

\noindent $\bullet$ \textbf{MSPLD}~\cite{dong2018few} adopts a similar setting as WL-FSOD, and the difference is that MSPLD simultaneously trains multiple deep detectors instead of only one traditional detector in WL-FSOD. MSPLD also excavates potential objects from the unlabeled dataset, and it proposes an alternating optimization strategy to update these multiple detectors. However, unlike standard FSOD methods that can handle the extreme low-shot condition~(one annotated sample for each category), MSPLD still requires much more annotations~(about $1 \%$ of entire images). Besides, this method cannot preserve the performance of previous models when adding new novel classes.

\subsection{Weakly-Supervised Few-Shot Object Detection\label{sec:weak_fsod_methods}}

Weakly-supervised Few-Shot Object Detection~(weakly-supervised FSOD) aims to incorporate ``image-level annotations''~(i.e., the classes presented in the images that can be obtained conveniently) into FSOD. Currently only a few methods delve into weakly-supervised FSOD: NOTE-RCNN~\cite{jiyanggaoNOTERCNN2019}, UniT~\cite{siddhesh2021unit}, vMF-MIL~\cite{Shaban2021fsweak}, and StarNet~\cite{LeonidStarNet2021}. Actually, these four methods adopt different weakly-supervised FSOD settings, which will be illustrated below.

\noindent $\bullet$ \textbf{NOTE-RCNN}~\cite{jiyanggaoNOTERCNN2019} expands the setting of standard FSOD by incorporating a large number of images with image-level annotations for novel classes. This method adopts a similar training strategy with semi-supervised FSOD methods, which iteratively excavates high-confidence potential objects and re-trains the model with them. The difference is that NOTE-RCNN only selects objects with the same pseudo-labels as the corresponding image-level annotations to train the newly added classification head. Besides, it adopts knowledge distillation to mitigate the overfitting problem.

\noindent $\bullet$ \textbf{UniT}~\cite{siddhesh2021unit}. Unlike NOTE-RCNN, UniT utilizes image-level annotations for base classes. Before the base training stage and the few-shot fine-tuning stage, UniT uses an OICR method~\cite{Peng2017Mul} to train a weakly-supervised object detector using image-level annotations. During few-shot fine-tuning, UniT additionally uses semantic similarity and visual similarity to capture similarities between base classes and novel classes, and uses them to transfer the predictions from base classes to novel classes. With the auxiliary image-level annotations and class semantic information, UniT outperforms many standard FSOD methods by a large margin.

\noindent $\bullet$ \textbf{vMF-MIL}~\cite{Shaban2021fsweak}. Different from NOTE-RCNN and UniT that retain a few bounding box annotations for novel classes, vMF-MIL proposes a more challenging setting that only image-level annotations are available for novel classes. This work proposes an EM-like algorithm to find a common object representation across a set of images containing a common novel object. It uses the obtained common object representations to select the potential objects for each category and finally trains a detector for novel classes with these selected samples.

\noindent $\bullet$ \textbf{StarNet}~\cite{LeonidStarNet2021} proposes the most challenging setting~(compared to existing methods) that uses only image-level annotations for both base classes and novel classes. Given only image-level annotations, StarNet calculates the matching score between two images by excavating the highly related regions of these images according to the spatial alignment their feature maps, and generates the classification scores based on the calculated matching scores.
Furthermore, StarNet also generates prototype for each class by accumulating the features of regions from the same class, and uses these class prototypes for classification.

\subsection{Incremental Few-Shot Object Detection\label{sec:incre_fsod_methods}}

Incremental Few-Shot Object Detection~(incremental FSOD) is another challenging setting of FSOD. In this setting, novel classes are registered incrementally with a few annotated samples during the novel testing stage. Incremental FSOD requires the model to detect newly added classes while simultaneously not forgetting the knowledge of old classes. Current incremental FSOD methods can also be categorized into \textbf{meta-learning methods} and \textbf{transfer-learning methods}.

\noindent $\bullet$ \textbf{Meta-Learning Methods.}
ONCE~\cite{PerezRuaZHXIncremental2020} is the earliest method for incremental FSOD~\cite{xingyiCentrenet2020} based on CenterNet. To support incremental learning, ONCE separates CenterNet into category-agnostic components and category-specific components.
ONCE first trains the entire model in the regular supervised way on the base dataset. Next, it adopts meta-learning to train a category-specific module to generate class codes for all classes, which will be used to generate classification scores.
ONCE is an early approach for incremental FSOD requiring no few-shot fine-tuning, but it suffers a severe performance drop compared with methods for standard FSOD.
Sylph~\cite{yin2022CVPR} improves ONCE in several aspects. Specifically, Sylph replaces the class-specific regression branch with a class-agnostic regression branch, and proposes a class-specific binary classifier with a weight normalization strategy to improve adaptation to newly added classes.

\noindent $\bullet$ \textbf{Transfer-Learning Methods.}
LEAST~\cite{pengyangliClassIncremental2021} tackles incremental FSOD based on transfer-learning. Similar to ONCE, LEAST separates Faster R-CNN into category-agnostic components and category-specific components.
LEAST trains the entire model in the base training stage, yet only optimizes the category-specific components in the few-shot fine-tuning stage. This optimization strategy removes the unnecessary weight adaptation of category-agnostic components and is expected to reduce training costs and generalize the model to novel classes.
As previous incremental learning methods, LEAST introduces knowledge distillation to retain the knowledge for the detection of base classes. Furthermore, LEAST proposes a clustering-based exemplar selection algorithm to select a few informative samples from the old training set for model fine-tuning. LEAST outperforms ONCE by a large margin on novel classes under the same incremental FSOD setting.
Incremental-DETR~\cite{dong2022incremental} is another transfer-learning method for incremental FSOD. It adopts DETR as the detection framework, and it also utilizes knowledge distillation to mitigate the catastrophic forgetting problem. Besides, it applies selective search to excavate novel objects and self-train the model with these mined objects, making the model generalize well to novel classes.

\subsection{Generalized Few-Shot Object Detection\label{sec:generalized_fsod_methods}}

\noindent $\bullet$ \textbf{Retentive R-CNN}~\cite{fan2021generalized}. Unlike other methods that only focus on the performance of the novel classes, Retentive R-CNN~\cite{fan2021generalized} proposes a generalized FSOD setting which aims to retain the performance on the base classes after fine-tuning.
To achieve this goal, it incorporates the knowledge of base classes into RoI classification component and RPN component of the fine-tuned model.
For the RoI classification component, this method uses a consistency loss between classification scores from the pre-trained model and the fine-tuned model to distill the knowledge of base classes into the fine-tuned model.
For the RPN component, Retentive R-CNN unfreezes the final layer for object prediction during fine-tuning, which is different from the original TFA. And this component computes the object prediction scores as the ensemble of outputs from the original model and the fine-tuned model.

\noindent $\bullet$ \textbf{CFA}~\cite{guirguis2022CVPR} finds that although Retentive R-CNN can mitigate the forgetting on the base classes, it drops the performance on the novel classes.
Therefore, CFA proposes a constraint-based fine-tuning method for the novel fine-tuning stage. Specifically, it preserves some images for each added class, and constrain that the detection loss on these preserved images not to increase while fine-tuning on the newly added data. To this end, it adopts A-GEM~\cite{riemer2019ICLR} to constrain that the angle between gradients on the old class and new class is acute.
With this fine-tuning strategy, CFA outperforms Retentive R-CNN by a large margin.

\subsection{Hierarchical Few-Shot Object Detection\label{sec:hierarchy_fsod_methods}}

\noindent $\bullet$ \textbf{HiCLPR}~\cite{park2022hierarchical}. Hierarchical Few-Shot Object Detection conducts FSOD in a hierarchical taxonomy. Recently, HiCLPR proposes a hierarchical FSOD benchmark on bird classification. HiCLPR organizes all bird categories into a 4-level hierarchical taxonomy system: order, family, genus and species, and divides the base and novel classes at the order level.
To tackle the 4-level hierarchical taxonomy problem, HiCLPR proposes a corresponding 4-level hierarchical classification head, where each level of the classification head is designed for the same level of the taxonomy system.
Besides, HiCLPR utilizes contrastive learning for feature learning and a probabilistic loss to encourage the child nodes to correct the misclassified samples of their parent nodes.

==> tables/soc_fsod_coco_benchmark.tex <==
\begin{table}
\footnotesize
\renewcommand\arraystretch{1.1}
\centering
\caption{\color{blue} Performance (mAP) of FSOD methods on the MS COCO benchmark~(only the methods with released codes are listed). These FSOD methods are evaluated under the $10, 30$-shot conditions. ${}^{\star}$ denotes that the results are averaged over multiple runs, and R-50 \& R-101 denote ResNet-50 \& ResNet-101.}
\label{tab:soc_coco_performance}
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{c|c|c| 
*6{c}} % 控制表格的格式
    \toprule
  ~ & \textbf{Method} & \textbf{Backbone} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{5} & \textbf{10} & \textbf{30} \\
  \midrule
  \multirow{13}*{\rotatebox{270}{\textbf{\small Meta-Learning}}} & FSRW~(2018) & YOLOv2 & N/A & N/A & N/A & N/A & 5.6 & 9.1 \\

~ & Meta-RCNN~(2019) & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 8.7 & 12.4 \\

~ & FsDet~(2020)${}^{\star}$ & Faster R-CNN~(R-101) & 4.5 & 6.6 & 7.2 & 10.7 & 12.5 & 14.7 \\

~ & Attention-RPN~(2020) & Faster R-CNN~(R-50) & 4.2 & 5.6 & 6.6 & 8.0 & 11.1 & 13.5 \\

~ & DRL~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 11.9 & 14.6 \\

~ & DCNet~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 12.8 & 18.6 \\

~ & CME~(2021) & YOLOv2 & N/A & N/A & N/A & N/A & 15.1 & 16.9 \\

~ & Meta-DETR~(2022)${}^{\star}$ & Def. DETR~(R-101) & 7.5 & N/A & 13.5 & 15.4 & 19.0 & 22.2 \\

~ & QA-FewDet~(2021) & Faster R-CNN~(R-101) & 4.9 & 7.6 & 8.4 & 9.7 & 11.6 & 16.5 \\

~ & DAnA-FasterRCNN~(2021) & Faster R-CNN~(R-50) & N/A & N/A & N/A & N/A & 18.6 & 21.6 \\

~ & Meta Faster R-CNN~(2022) & Faster R-CNN~(R-101) & 5.1 & 7.6 & 9.8 & 10.8 & 12.7 & 16.6 \\

~ & FCT~(2022)${}^{\star}$ & Faster R-CNN~(PVTv2-B2-Li) & 5.1 & 7.2 & 9.8 & 12.0 & 15.3 & 20.2 \\

~ & VFA~(2023) & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 16.2 & 18.9 \\

\hline

\multirow{14}*{\rotatebox{270}{\textbf{\small Transfer-Learning}}} & TFA w/cos~(2020) & Faster R-CNN~(R-101) & 3.4 & 4.6 & 6.6 & 8.3 & 10.0 & 13.7 \\

~ & Halluc~(2021) & Faster R-CNN~(R-101) & 4.4 & 5.6 & 7.2 & N/A & N/A & N/A \\

~ & MPSR~(2020) & Faster R-CNN~(R-101) & 2.3 & 3.5 & 5.2 & 6.7 & 9.8 & 14.1 \\

% ~ & LEAST~(2021)${}^{\star}$~\cite{pengyangliClassIncremental2021} & ~ & N/A & N/A & N/A & N/A & 12.8 & N/A \\

~ & ${\rm FSOD}^{\rm up}~(2021)$ & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 11.0 & 15.6 \\

~ & FSCE~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 11.9 & 16.4 \\

~ & DeFRCN~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & 4.8 & 8.5 & 10.7 & 13.6 & 16.8 & 21.2 \\

~ & N-PME~(2022) & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 10.6 & 14.1 \\

~ & FSOD-KI~(2022) & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 13.0 & 16.8 \\

~ & FSOD-KD~(2022) & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 12.5 & 17.1 \\

~ & FADI~(2022) & Faster R-CNN~(R-101) & N/A & N/A & N/A & N/A & 12.2 & 16.1 \\

~ & PSEUDO~(2022) & Faster R-CNN~(Swin-S) & N/A & N/A & N/A & N/A & 19.0 & 26.8 \\

~ & FSOD-DIS~(2022) & Faster R-CNN~(R-101) & 10.8 & 13.9 & 15.0 & 16.4 & 19.4 & 22.7 \\

~ & imTED~(2022) & Faster R-CNN~(ViT-B) & N/A & N/A & N/A & N/A & 22.5 & 30.2 \\

~ & DETReg~(2022) & Def. DETR~(R-50) & N/A & N/A & N/A & N/A & 25.0 & 30.0 \\
  \bottomrule
  \end{tabular}}
\end{table}

==> tables/soc_fsod_pascal_avg_benchmark.tex <==
\begin{table}
\footnotesize
\renewcommand\arraystretch{1.1}
\centering
\caption{\color{blue} Performance~(mAP50) of FSOD methods on the PASCAL VOC benchmark~(only the methods with released codes are listed). These FSOD methods are evaluated on the PASCAL VOC dataset under the $1, 2, 3, 5, 10$-shot condition. The results are averaged over three splits of base \& novel classes. For each shot, the red font denotes the best performance, and the gray font denotes the second-best performance. ${}^{\star}$ denotes that the results are averaged over multiple runs, and R-101 denotes ResNet-101.}
\label{tab:soc_pascalvoc_avg_performance}
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{c|c|c|
*5{c}} % 控制表格的格式
    \toprule
  \multirow{2}*{} & \multirow{2}*{\textbf{Method}} & \multirow{2}*{\textbf{Detector~(Backbone)}} & \multicolumn{5}{c}{\textbf{3 Novel Sets~(Averaged)}} \\
  ~ & ~ & ~ & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{5} & \textbf{10} \\
  \midrule

\multirow{9}*{\rotatebox{270}{\textbf{Meta-Learning}}}  &  FSRW~(2018)  &  YOLOv2  & 17.3 & 18.8 & 25.9 & 35.6 & 44.5 \\
~  &  Meta-RCNN~(2019)  &  Faster R-CNN~(R-101)  & 14.9 & 21.0 & 30.7 & 40.6 & 48.3 \\
~  &  FsDet~(2020)${}^{\star}$  &  Faster R-CNN~(R-101)  & 22.3 & 30.0 & 37.1 & 43.3 & 50.9 \\
~  &  DRL~(2021)${}^{\star}$  &  Faster R-CNN~(R-101)  & 25.8 & 35.4 & 41.3 & 42.3 & 53.6 \\
~  &  DCNet~(2021)${}^{\star}$  &  Faster R-CNN~(R-101)  & 29.8 & 32.4 & 38.0 & 43.5 & 52.3 \\
~  &  CME~(2021)  &  YOLOv2  & 15.4 & 23.6 & 29.8 & 41.1 & 45.4 \\
~  &  Meta-DETR~(2022)${}^{\star}$  &  Def. DETR~(R-101)  & 32.6 & 41.0 & 46.2 & 51.6 & 57.3 \\
~  &  QA-FewDet~(2021)  &  Faster R-CNN~(R-101)  & 34.5 & 44.2 & 50.0 & 55.4 & 56.0 \\
% ~  &  FCT~(2022)${}^{\star}$  &  {\scriptsize Faster R-CNN~(PVTv2-B2-Li)}  & 33.0 & 42.6 & 47.6 & 52.6 & 56.0 \\
~  &  VFA~(2023)  &  Faster R-CNN~(R-101)  & 49.3 & {\color{gray} 55.2} & {\color{gray} 57.5} & 59.3 & 59.3 \\
\hline
\multirow{11}*{\rotatebox{270}{\textbf{Transfer-Learning}}}  &  TFA w/cos~(2020)  &  Faster R-CNN~(R-101)  & 31.4 & 32.6 & 40.5 & 46.8 & 48.3 \\
~  &  Halluc~(2021)  &  Faster R-CNN~(R-101)  & 37.9 & 39.6 & 42.4 & 47.8 & 48.5 \\
~  &  MPSR~(2020)  &  Faster R-CNN~(R-101)  & 33.9 & N/A & 44.3 & 47.7 & 53.1 \\
~  &  ${\rm FSOD}^{\rm up}(2021)$  &  Faster R-CNN~(R-101)  & 36.8 & 39.3 & 45.1 & 49.4 & 54.5 \\
~  &  FSCE~(2021)${}^{\star}$  &  Faster R-CNN~(R-101)  & 26.4 & 36.0 & 41.6 & 48.7 & 54.1 \\
~  &  DeFRCN~(2021)${}^{\star}$  &  Faster R-CNN~(R-101)  & 34.9 & 43.9 & 51.5 & 56.5 & 60.0 \\
~  &  FSOD-KI~(2022)  &  Faster R-CNN~(R-101)  & {\color{gray} 50.2} & 54.7 & 57.4 & {\color{gray} 60.2} & {\color{gray} 61.0} \\
~  &  FSOD-KD~(2022)  &  Faster R-CNN~(R-101)  & 39.3 & 44.4 & 47.5 & 52.8 & 54.2 \\
~  &  FADI~(2022)  &  Faster R-CNN~(R-101)  & 42.2 & 46.5 & 47.9 & 52.4 & 56.9 \\
~  &  PSEUDO~(2022)  &  Faster R-CNN~(R-101)  & 45.2 & 45.0 & 54.8 & 57.5 & 58.6 \\
~  &  FSOD-DIS~(2022)  &  Faster R-CNN~(R-101)  & \textbf{\color{red} 53.9} & \textbf{\color{red} 57.0} & \textbf{\color{red} 60.0} & \textbf{\color{red} 62.3} & \textbf{\color{red} 61.9} \\

\bottomrule
\end{tabular}}
\end{table}

==> tables/soc_fsod_pascal_benchmark.tex <==
\begin{table}
\footnotesize
\renewcommand\arraystretch{1.1}
\centering
\caption{\color{blue} Performance~(mAP50) of FSOD methods on the PASCAL VOC benchmark~(only the methods with released codes are listed). These FSOD methods are evaluated on the three splits of PASCAL VOC dataset under the $1, 2, 3, 5, 10$-shot condition. For each shot, the red font denotes the best performance, and the gray font denotes the second-best performance. ${}^{\star}$ denotes that the results are averaged over multiple runs, and R-101 denotes ResNet-101.}
\label{tab:soc_pascalvoc_performance}
\setlength{\tabcolsep}{0.15mm}{
\begin{tabular}{c|c|c|
*5{c}|*5{c}|*5{c}} % 控制表格的格式
    \toprule
  \multirow{2}*{} & \multirow{2}*{\textbf{Method}} & \multirow{2}*{\textbf{Detector~(Backbone)}} & \multicolumn{5}{c|}{\textbf{Novel Set 1}} &  \multicolumn{5}{c|}{\textbf{Novel Set 2}} & \multicolumn{5}{c}{\textbf{Novel Set 3}} \\
  ~ & ~ & ~ & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{5} & \textbf{10} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{5} & \textbf{10} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{5} & \textbf{10} \\
  \midrule

\multirow{9}*{\rotatebox{270}{\textbf{Meta-Learning}}} & FSRW~(2018) & YOLOv2 & 14.8 & 15.5 & 26.7 & 33.9 & 47.2 & 15.7 & 15.3 & 22.7 & 30.1 & 40.5 & 21.3 & 25.6 & 28.4 & 42.8 & 45.9 \\

~ & Meta-RCNN~(2019) & Faster R-CNN~(R-101) & 19.9 & 25.5 & 35.0 & 45.7 & 51.5 & 10.4 & 19.4 & 29.6 & 34.8 & 45.4 & 14.3 & 18.2 & 27.5 & 41.2 & 48.1 \\

~ & FsDet~(2020)${}^{\star}$ & Faster R-CNN~(R-101) & 24.2 & 35.3 & 42.2 & 49.1 & 57.4 & 21.6 & 24.6 & 31.9 & 37.0 & 45.7 & 21.2 & 30.0 & 37.2 & 43.8 & 49.6 \\

~ & DRL~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & 30.3 & 40.8 & 49.1 & 48.0 & 58.6 & 22.4 & 36.1 & 36.9 & 35.4 & 51.8 & 24.8 & 29.3 & 37.9 & 43.6 & 50.4 \\

~ & DCNet~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & 33.9 & 37.4 & 43.7 & 51.1 & 59.6 & 23.2 & 24.8 & 30.6 & 36.7 & 46.6 & 32.3 & 34.9 & 39.7 & 42.6 & 50.7 \\

~ & CME~(2021) & YOLOv2 & 17.8 & 26.1 & 31.5 & 44.8 & 47.5 & 12.7 & 17.4 & 27.1 & 33.7 & 40.0 & 15.7 & 27.4 & 30.7 & 44.9 & 48.8 \\

~ & Meta-DETR~(2022)${}^{\star}$ & Def. DETR~(R-101) & 35.1 & 49.0 & 53.2 & 57.4 & 62.0 & 27.9 & 32.3 & 38.4 & 43.2 & 51.8 & 34.9 & 41.8 & 47.1 & 54.1 & 58.2 \\

~ & QA-FewDet~(2021) & Faster R-CNN~(R-101) & 42.4 & 51.9 & 55.7 & 62.6 & 63.4 & 25.9 & 37.8 & 46.6 & 48.9 & 51.1 & 35.2 & 42.9 & 47.8 & 54.8 & 53.5 \\

% ~ & Meta Faster R-CNN~(2022)~\cite{guangxingMetaFaster2021} & 43.0 & 54.5 & 60.6 & 66.1 & 65.4 & 27.7 & 35.5 & 46.1 & 47.8 & 51.4 & 40.6 & 46.4 & 53.4 & 59.9 & 58.6 \\

% ~ & FCT~(2022)${}^{\star}$ & {\scriptsize Faster R-CNN~(PVTv2-B2-Li)} & 38.5 & 49.6 & 53.5 & 59.8 & 64.3 & 25.9 & 34.2 & 40.1 & 44.9 & 47.4 & 34.7 & 43.9 & 49.3 & 53.1 & 56.3 \\

% ~ & Hierarchy-FasterRCNN~(2022)~\cite{park2022hierarchical} & 58.6 & 61.0 & 62.5 & 63.7 & 64.9 & 38.9 & 47.6 & 49.0 & 51.7 & 53.6 & 52.9 & 57.1 & 55.6 & 59.6 & 60.7 \\

~ & VFA~(2023) & Faster R-CNN~(R-101) & {\color{gray} 57.7} & {\color{gray} 64.6} & {\color{gray} 64.7} & {\color{gray} 67.2} & 67.4 & 41.4 & {\color{gray} 46.2} & {\color{gray} 51.1} & 51.8 & 51.6 & 48.9 & 54.8 & 56.6 & 59.0 & 58.9 \\
\hline

% \multirow{11}*{Transfer-Learning} & \\

\multirow{11}*{\rotatebox{270}{\textbf{Transfer-Learning}}} & TFA w/cos~(2020) & Faster R-CNN~(R-101) & 39.8 & 36.1 & 44.7 & 55.7 & 56.0 & 23.5 & 26.9 & 34.1 & 35.1 & 39.1 & 30.8 & 34.8 & 42.8 & 49.5 & 49.8 \\

% ~ & Halluc~(2021)~\cite{zhang2021hallucination} & 47.0 & 44.9 & 46.5 & 54.7 & 54.7 & 26.3 & 31.8 & 37.4 & 37.4 & 41.2 & 40.4 & 42.1 & 43.3 & 51.4 & 51.4 \\

~ & Halluc~(2021) & Faster R-CNN~(R-101) & 47.0 & 44.9 & 46.5 & 54.7 & 54.7 & 26.3 & 31.8 & 37.4 & 37.4 & 41.2 & 40.4 & 42.1 & 43.3 & 51.4 & 49.6 \\

~ & MPSR~(2020) & Faster R-CNN~(R-101) & 41.7 & N/A & 51.4 & 55.2 & 61.8 & 24.4 & N/A & 39.2 & 39.9 & 47.8 & 35.6 & N/A & 42.3 & 48.0 & 49.7 \\

~ & ${\rm FSOD}^{\rm up}(2021)$ & Faster R-CNN~(R-101) & 43.8 & 47.8 & 50.3 & 55.4 & 61.7 & 31.2 & 30.5 & 41.2 & 42.2 & 48.3 & 35.5 & 39.7 & 43.9 & 50.6 & 53.5 \\

~ & FSCE~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & 32.9 & 44.0 & 46.8 & 52.9 & 59.7 & 23.7 & 30.6 & 38.4 & 46.0 & 48.5 & 22.6 & 33.4 & 39.5 & 47.3 & 54.0 \\

~ & DeFRCN~(2021)${}^{\star}$ & Faster R-CNN~(R-101) & 40.2 & 53.6 & 58.2 & 63.6 & 66.5 & 29.5 & 39.7 & 43.4 & 48.1 & {\color{gray} 52.8} & 35.0 & 38.3 & 52.9 & 57.7 & 60.8 \\

~ & FSOD-KI~(2022) & Faster R-CNN~(R-101) & 57.0 & 62.3 & 63.3 & 66.2 & {\color{gray} 67.6} & \textbf{\color{red} 42.8} & 44.9 & 50.5 & {\color{gray} 52.3} & 52.2 & {\color{gray} 50.8} & {\color{gray} 56.9} & {\color{gray} 58.5} & {\color{gray} 62.1} & {\color{gray} 63.1} \\

~ & FSOD-KD~(2022) & Faster R-CNN~(R-101) & 46.7 & 53.1 & 53.8 & 61.0 & 62.1 & 30.1 & 34.2 & 41.6 & 41.9 & 44.8 & 41.0 & 46.0 & 47.2 & 55.4 & 55.6 \\

~ & FADI~(2022) & Faster R-CNN~(R-101) & 50.3 & 54.8 & 54.2 & 59.3 & 63.2 & 30.6 & 35.0 & 40.3 & 42.8 & 48.0 & 45.7 & 49.7 & 49.1 & 55.0 & 59.6 \\

~ & PSEUDO~(2022) & Faster R-CNN~(R-101) & 54.5 & 53.2 & 58.8 & 63.2 & 65.7 & 32.8 & 29.2 & 50.7 & 49.8 & 50.6 & 48.4 & 52.7 & 55.0 & 59.6 & 59.6 \\

~ & FSOD-DIS~(2022) & Faster R-CNN~(R-101) & \textbf{\color{red} 63.4} & \textbf{\color{red} 66.3} & \textbf{\color{red} 67.7} & \textbf{\color{red} 69.4} & \textbf{\color{red} 68.1} & {\color{gray} 42.1} & \textbf{\color{red} 46.5} & \textbf{\color{red} 53.4} & \textbf{\color{red} 55.3} & \textbf{\color{red} 53.8} & \textbf{\color{red} 56.1} & \textbf{\color{red} 58.3} & \textbf{\color{red} 59.0} & \textbf{\color{red} 62.2} & \textbf{\color{red} 63.7} \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/soc_osol_benchmark.tex <==
\begin{table}
\footnotesize
\renewcommand\arraystretch{1.1}
\centering
\caption{\color{blue} Performance~(mAP50) of OSOL methods on novel classes. On each benchmark, the red font denotes the best performance, and the gray font denotes the second-best performance. Note that PASCAL VOC has only one class split, while the results on MS COCO are averaged over four different class splits. R-50 \& R-101 denotes ResNet-50 \& ResNet-101.}
\label{tab:soc_osod_performance}
\setlength{\tabcolsep}{1.mm}{
\begin{tabular}{ c
*4{c}} % 控制表格的格式
    \toprule
  \textbf{Type} & \textbf{Method} & \textbf{Detector~(Backbone)} & \textbf{PASCAL VOC} & \textbf{MS COCO} \\
  \midrule
\multirow{2}*{Object Tracking Methods} & SiamFC~(2018) & SNet \& ENet~(VGG-16) & 13.3 & N/A \\
~ & SiamRPN~(2018) & Faster R-CNN~(AlexNet) & 14.2 & N/A \\

\hline

\multirow{4}*{Concatenation-Based Methods} & SiamMask~(2019) & Faster R-CNN~(R-50) & N/A & 16.8 \\

~ & OSCD~(2020) & Faster R-CNN~(AlexNet) & 52.1 & N/A \\

~ & OSOLwT~(2020) & Faster R-CNN~(R-50) & 69.1 & N/A \\

~ & FOC OSOL~(2021) & Faster R-CNN~(R-50) & 71.0 & N/A \\

\hline

\multirow{8}*{Attention-Based Methods} & CoAE~(2019) & Faster R-CNN~(R-50) & 68.2 & 22.0 \\

~ & ADA OSOL~(2022) & Faster R-CNN~(R-50) & 72.3 & 23.6 \\

~ & AUG OSOL~(2022) & Faster R-CNN~(R-50) & 73.2 & 23.9 \\

~ & AIT~(2021) & Faster R-CNN~(R-50) & 73.1 & 24.3 \\

~ & BHRL~(2022) & Faster R-CNN~(R-50) & 73.8 & \textbf{\color{red} 25.6} \\

~ & SaFT~(2022) & FCOS~\cite{tian2019FSOS}~(R-101) & 74.5 & {\color{gray} 24.9} \\

~ & CAT~(2021) & Faster R-CNN~(R-50) & \textbf{\color{red} 75.5} & 24.4 \\

~ & ABA OSOL~(2023) & Faster R-CNN~(R-50) & {\color{gray} 74.6} & 23.6 \\

\bottomrule
\end{tabular}}
\end{table}
